Programming with Permissions in Mezzo

We present Mezzo, a typed programming language of ML lineage. Mezzo is equipped with a novel static discipline of duplicable and affine permissions, which controls aliasing and ownership. This rules out certain mistakes, including representation exposure and data races, and enables new idioms, such as gradual initialization, memory re-use, and (type)state changes. Although the core static discipline disallows sharing a mutable data structure, Mezzo offers several ways of working around this restriction, including a novel dynamic ownership control mechanism which we dub "adoption and abandon".

==> Makefile <==
# ----------------------------------------------------------------------------
# Set any paper-specific variables.

include Makefile.local

# ----------------------------------------------------------------------------
# Eliminate the default known suffixes.

.SUFFIXES:

# ----------------------------------------------------------------------------
# Definitions.

PSPROLOGUE := \nonstopmode\input
PROLOGUE   := \def\fppdf{true}\nonstopmode\input
FPLONG     := \\\\def\\\\fplong{true}

# ----------------------------------------------------------------------------
# Generic rules.

%.pdf: $(wildcard *.tex) $(wildcard *.sty) $(wildcard *.bib) $(wildcard ../common/*.tex) $(wildcard ../common/*.bib)
	pdflatex "$(PROLOGUE)" $(DOC).tex
	bibtex $(DOC)
	pdflatex "$(PROLOGUE)" $(DOC).tex
	pdflatex "$(PROLOGUE)" $(DOC).tex

%.ps: $(wildcard *.tex) $(wildcard *.sty) $(wildcard *.bib) $(wildcard ../common/*.tex) $(wildcard ../common/*.bib)
	latex "$(PSPROLOGUE)" $(DOC).tex
	bibtex $(DOC)
	latex "$(PSPROLOGUE)" $(DOC).tex
	latex "$(PSPROLOGUE)" $(DOC).tex
	dvips -e 0 -t letter $(DOC).dvi

# ----------------------------------------------------------------------------
# Targets.

.PHONY: pdf ps clean log export

pdf: $(DOC).pdf

ps: $(DOC).ps

clean::
	rm -f *.aux *.log *.bbl *.blg *~ *.out *.thm *.cb *.cb2
	rm -f $(DOC).dvi $(DOC).pdf

log: pdf
	./decrypt.sh $(DOC).log

# ----------------------------------------------------------------------------
# Short and long versions.

long:
	rm -f switch.tex
	echo "$(FPLONG)" > switch.tex
	$(MAKE) pdf

short:
	rm -f switch.tex
	touch switch.tex
	$(MAKE) pdf

# ----------------------------------------------------------------------------
# Web export.

WWW   := yquem.inria.fr:public_html/publis
SHORT := pottier-protzenko-mezzo.pdf
LONG  := mezzo-icfp2013-long.pdf

export:
#	$(MAKE) clean short
#	scp -p -B -C $(DOC).pdf $(WWW)/$(SHORT)
	$(MAKE) clean long
	scp -p -B -C $(DOC).pdf $(WWW)/$(LONG)


==> courte-ou-longue.tex <==
\makeatletter
\IfFileExists{switch.tex}{
  \input{switch.tex}
  \@ifundefined{fplong}{
  \newenvironment{courte}{}{}
  \newenvironment{longue}{\comment}{\endcomment}
  }{
  \@ifundefined{WhizzyTeX}{\usepackage[pdftex]{changebar}}{\usepackage[dvips]{changebar}}
  \newenvironment{courte}{\comment}{\endcomment}
  \newenvironment{longue}{}{}
  }
}{}
\makeatother


==> figure-mlist.tex <==
\begin{figure}[t]
\begin{lstlisting}
val rec concatAux [a] (
      xs: MCons { head: a; tail: mlist a },
      consumes ys: mlist a) : () =
  match xs.tail with
  | MNil  -> xs.tail <- ys
  | MCons -> concatAux (xs.tail, ys)
  end

val concat [a] (
    consumes xs: mlist a,
    consumes ys: mlist a) : mlist a =
  match xs with
  | MNil  -> ys
  | MCons -> concatAux (xs, ys); xs
  end
\end{lstlisting}
\caption{Concatenation of mutable lists} % (tail-recursive version)
\label{fig:mlist}
\end{figure}


==> figure-translate-consumes.tex <==

  \begin{figure*}
    \begin{center}
      \begin{mathpar}
        \inferrule
        {t_1 \text{ contains no name introductions }\\
         t_{1,l} = [\tau/\tyconsumes\tau]t_1\\
         t_{1,r} = [\top/\tyconsumes\tau]t_1}
        {\tyearrow{t_1}{t_2} \vartriangleright
           \tyforall{r}{\kterm}{
             \tyarrow{
               \tybar{
                 \tysingleton{r}
               }{
                 \tyatomic{r}{t_{1,l}}
               }
             }{
               \tybar{
                 t_2
               }{
                 \tyatomic{r}{t_{1,r}}
               }
             }
           }
        }
      \end{mathpar}
    \end{center}
    \caption{Translating consumes annotations}
    \label{fig:translation-consumes}
  \end{figure*}



==> macros.tex <==
\makeatletter

\newcommand{\mezzo}{%
  \texorpdfstring{%
    \protect\mbox{%
      \protect\textit{\protect\textsf{%
        Me\protect\raisebox{-.1ex}z\protect\hspace{-.3ex}{\protect\raisebox{.2ex}z}\protect\hspace{-.1ex}o%
      }}%
    }%
  }{Mezzo}\xspace
}

\newcommand{\hamlet}{\mezzo}
\newcommand{\ocaml}{OCaml\xspace}

\@ifpackageloaded{listings}{
  \lstset{
    language=caml,
    flexiblecolumns=false,
    showstringspaces=false,
    basicstyle=\tt\small,
    framesep=5pt,
    numberstyle=\tiny,
    numbersep=5pt,
    escapeinside={--}{\^^M},
    morekeywords={data,val,consumes,adopts,take,give,from},
  }
  \def\li{\lstinline}
  \def\qli|#1|{``\li|#1|''}
  \def\sqli|#1|{``\texttt{\small #1}''}

}

\@ifpackageloaded{tikz}{

  \newcommand{\inlinetikzbox}[2]{%
    \tikz[baseline]{%
      \node[fill=gray!20,anchor=base] (#1) {#2};%
    }%
  }

  \AtBeginDocument{\tikzstyle{every picture}+=[remember picture]}
}{}



\@ifpackageloaded{color}{
  \definecolor{mygrey}{rgb}{0.9,0.9,0.9}
  \newcommand{\mystrut}{\rule[-.1\baselineskip]{0pt}{.65\baselineskip}}
  \newcommand{\shaded}[1]{\colorbox{mygrey}{$\mystrut\smash{#1}$}}
}{}

\makeatother


\newcommand{\kw}[1]{\ensuremath{\text{\textsf{#1}}}}
\newcommand{\ktype}{\ensuremath{\kw{type}}}
\newcommand{\kterm}{\kw{term}}
\newcommand{\kperm}{\kw{perm}}

\newcommand{\kreset}{\kw{extend}}
\newcommand{\kleft}{\kw{left}}
\newcommand{\kright}{\kw{right}}
\newcommand{\khead}{\kw{head}}
\newcommand{\ktail}{\kw{tail}}
\newcommand{\ktrue}{\kw{true}}
\newcommand{\kfalse}{\kw{false}}

\newcommand{\kconsumes}{\kw{consumes}}

\makeatletter
\@ifundefined{mode}{
  \newcommand{\mode}[1]{\ensuremath{m\,#1}}
}{}
\makeatother

\newcommand{\moded}{\kw{duplicable}}
\newcommand{\modex}{\kw{exclusive}}
\newcommand{\modea}{\kw{affine}}

\newcommand{\fhead}{\kw{head}}
\newcommand{\ftail}{\kw{tail}}
\newcommand{\nret}{\kw{ret}}

\newcommand{\tyvar}                   {a} % variable of kind type
\newcommand{\tyunknown}               {\kw{unknown}}
\newcommand{\tydynamic}               {\kw{dynamic}}
\newcommand{\tydynamicprime}[1]       {\kw{dynamic}'\,#1}
\newcommand{\tyarrow}[2]              {\ensuremath{#1 \rightarrow #2}}
\newcommand{\tyearrow}[2]              {\ensuremath{#1 \rightsquigarrow #2}}
\newcommand{\tytuple}[1]              {\ensuremath{(#1)}}
\newcommand{\tyconcretezero}[1]   {\ensuremath{\kw{#1}}}
\newcommand{\tyconcrete}[2]   {\ensuremath{\kw{#1}\,\{ #2 \}}}
\newcommand{\tyconcretev}[2]   {\ensuremath{\vec{\kw{#1}}\,\{ #2 \}}}
\newcommand{\tyconcreteadopts}[3]   {\ensuremath{\kw{#1}\,\{ #2 \}\,\kw{adopts}\,#3}}
\newcommand{\tyapp}[2]                {\ensuremath{#1\ #2}}
\newcommand{\tynameintro}[2]          {\ensuremath{#1: #2}}
\newcommand{\tyconsumes}[1]           {\ensuremath{\kw{consumes}\ #1}}
\newcommand{\tyforall}[3]             {\ensuremath{\forall(#1: #2)\ #3}}
\newcommand{\tyexists}[3]             {\ensuremath{\exists(#1: #2)\ #3}}
\newcommand{\tyforalln}[2]            {\ensuremath{[#1]\;#2}}
\newcommand{\tybar}[2]                {\ensuremath{(#1\mid#2)}}
\newcommand{\tysingleton}[1]{\raisebox{0.0mm}{\mbox{\kw{=}}}#1}
\newcommand{\tyand}[2]                {\tybar{#1}{#2}}
\newcommand{\tyimplies}[2]            {\ensuremath{#1 \Rightarrow #2}}
\newcommand{\tyempty}                 {\kw{empty}}
\newcommand{\tystar}[2]               {\ensuremath{#1 \ast #2}}
\newcommand{\tyatomic}[2] {\ensuremath{#1\,@\ #2}}

\newcommand{\tyint}                   {\kw{int}}
\newcommand{\tystring}                {\kw{string}}
\newcommand{\tyref}[1]                {\kw{ref}\;#1}
\newcommand{\tylist}[1]               {\kw{list}\;#1}
\newcommand{\tymlist}[1]              {\kw{mlist}\;#1}
\newcommand{\tymtree}[1]              {\kw{mtree}\;#1}
\newcommand{\typackage}[2]            {\tybar{\tysingleton{#1}}{\tyatomic{#1}{#2}}}

\newcommand{\econstraint}[2]          {\ensuremath{#1\!: #2}}
\newcommand{\equalified}[2]           {\ensuremath{#1\!\!::\!\!#2}}
\newcommand{\elet}[3]                 {\ensuremath{\kw{let}\ #1=#2\ \kw{in}\ #3}}
\newcommand{\efun}[3]                 {\ensuremath{\kw{fun}\ #1:#2=#3}}
\newcommand{\elambda}[4]              {\ensuremath{\lambda(#1:#2)\!: #3.\ #4}}
\newcommand{\eLambda}[3]              {\ensuremath{\Lambda(#1:#2).\ #3}}
\newcommand{\eassign}[3]              {\ensuremath{#1.#2 \leftarrow #3}}
\newcommand{\eassigntag}[2]           {\ensuremath{\kw{tag of}\ #1 \leftarrow \kw{#2}}}
\newcommand{\eaccess}[2]              {\ensuremath{#1.#2}}
\newcommand{\eassert}[1]              {\ensuremath{\kw{assert}\ #1}}
\newcommand{\eapply}[2]               {\ensuremath{#1\ #2}}
\newcommand{\etapply}[2]              {\ensuremath{#1\ [#2]}}
\newcommand{\ematch}[2]               {\ensuremath{\kw{match}\ #1\ \kw{with}\ #2}}
\newcommand{\pbranch}[2]              {\ensuremath{\,|\ #1 \rightarrow #2}}
\newcommand{\etuple}[1]               {\ensuremath{(#1)}}
\newcommand{\econstruct}[2]           {\ensuremath{\kw{#1}\,\{ #2 \}}}
\newcommand{\eifthenelse}[3]          {\ensuremath{\kw{if}\ #1\ \kw{then}\ #2\ \kw{else}\ #3}}
\newcommand{\esequence}[2]            {\ensuremath{#1;\ #2}}
\newcommand{\egive}[2]                {\ensuremath{\kw{give}\ #1\ \kw{to}\ #2}}
\newcommand{\etake}[2]                {\ensuremath{\kw{take}\ #1\ \kw{from}\ #2}}
\newcommand{\eowns}[2]                {\ensuremath{#1\ \kw{owns}\ #2}}
\newcommand{\efail}                   {\kw{fail}}


\newcommand{\subsub}{\equiv} % we could also use \lessgtr
\newcommand{\tynest}[2]{#1\prec#2}
\newcommand{\tylock}[1]{\kw{lock}\;#1}

\newcommand{\vdashw}{\vdash_\vartriangleright}
\newcommand{\vdashb}{\vdash_\blacktriangleright}

\newcommand{\modeD}[1]{\ensuremath{#1\text{ is duplicable}}}
\newcommand{\modeX}[1]{\ensuremath{#1\text{ is exclusive}}}
\newcommand{\modeA}[1]{\ensuremath{#1\text{ is affine}}}

\newcommand{\kmodeD}{\kw{duplicable}}
\newcommand{\kmodeX}{\kw{exclusive}}
\newcommand{\kmodeA}{\kw{affine}}

\newcommand{\osf}{\multimap} % from amssymb
\def\etal.{\emph{et al.}}

